GEXIA: Granularity Expansion and Iterative Approximation for Scalable Multi-grained Video-language Learning

In various video-language learning tasks, the challenge of achieving cross-modality alignment with multi-grained data persists. We propose a method to tackle this challenge from two crucial perspectives: data and modeling. Given the absence of a multi-grained video-text pretraining dataset, we introduce a Granularity EXpansion (GEX) method with Integration and Compression operations to expand the granularity of a single-grained dataset. To better model multi-grained data, we introduce an Iterative Approximation Module (IAM), which embeds multi-grained videos and texts into a unified, low-dimensional semantic space while preserving essential information for cross-modal alignment. Furthermore, GEXIA is highly scalable with no restrictions on the number of video-text granularities for alignment. We evaluate our work on three categories of video tasks across seven benchmark datasets, showcasing state-of-the-art or comparable performance. Remarkably, our model excels in tasks involving long-form video understanding, even though the pretraining dataset only contains short video clips.

==> sec/tables/ablation.tex <==
\begin{table*}[!t]
\centering
\caption{Ablation study results on different setups of pretraining data, encoder weight, the iteration number, and LLM assessment. The bolded text denotes the best comparable results.}
\vspace{-.3cm}
\footnotesize
    \subfloat[Text-to-video and Video-to-text results on ActivityNet Captions dataset with different pretraining data setups.]
    {
    \scalebox{0.9}{
        \begin{tabular}{l|ccc|ccc}
        \hlineB{3}
        \multirow{2}{*}{Data Setup} & \multicolumn{3}{c|}{T2V} & \multicolumn{3}{c}{V2T}\\
                                 & R@1 & R@5 & R@10 & R@1 & R@5 & R@10  \\ \hline
        SVST                                                                          &41.6     & 72.8     & 83.7      & 41.2     & 72.6     & 84.0       \\ 
        +LVLT                                                                   & 42.8     & 72.8     & 84.0      & 41.8     & 73.0     & 84.3         \\
                                                                                      
        +LVST                                                              & \textbf{43.1}     & \textbf{73.2}     & \textbf{84.5}     & \textbf{42.6}     & \textbf{73.4}     & \textbf{84.8}        \\ \hlineB{3}
        \end{tabular}
    } \label{ablation_data}
    }\hfill
    \subfloat[Text-to-video and Video-to-text results on ActivityNet Captions dataset with different encoder weight setups.]
    {
    \scalebox{0.9}{
    \begin{tabular}{l|ccc|ccc}
    \hlineB{3}
    \multirow{2}{*}{Encoder Weight Setup} & \multicolumn{3}{c|}{T2V} & \multicolumn{3}{c}{V2T}\\
                         & R@1 & R@5 & R@10 & R@1 & R@5 & R@10  \\ \hline
Scratch                  & 24.7     & 51.1     & 64.1      & 24.7     & 52.6     & 65.9       \\ 
Freeze CLIP       & 37.5     & 67.4     & 80.6      & 36.9     & 68.0     & 80.9         \\                 
Unfreeze CLIP & \textbf{45.3}     & \textbf{76.5}     & \textbf{86.6}     & \textbf{44.5}     &      \textbf{76.4}     & \textbf{87.3}        \\
    \hlineB{3}
    \end{tabular}
    } \label{ablation_encoder}
    }\hfill
    \subfloat[Retrieval results on the number of iterations across different datasets and scenarios, finetuning (FT) and zero-shot (ZS). A-Net: ActivityNet Captions; C-Ego: Charades-Ego.]
    {
    \scalebox{1}{
    \begin{tabular}{c|ccc|ccc|ccc|ccc|c}
\hlineB{3}
$\#iter$ & \multicolumn{3}{c|}{FT A-Net T2V} & \multicolumn{3}{c|}{FT A-Net V2T} & \multicolumn{3}{c|}{ZS MSRVTT T2V} & \multicolumn{3}{c|}{ZS LSMDC T2V} & ZS C-Ego\\
Video-Text                   & R@1 & R@5 & R@10 & R@1 & R@5 & R@10  &R@1 & R@5 & R@10 &R@1 & R@5 & R@10 &mAP \\ \hline
1-1                      & 43.1     & 73.2     & 84.5     & 42.6     & 73.4     & 84.8  & \textbf{37.3} &\textbf{63.8} & \textbf{72.5} &12.9 & \textbf{28.3} & \textbf{35.5} &22.9 \\ 
3-1                      & 44.8     & 75.5     & 86.0 & 44.7 & 75.4     & 86.5  & 36.3 &62.5 & 72.1 &13.8 & 27.7 & 35.3 &   \textbf{23.4}  \\       
3-3                      & \textbf{45.3}& \textbf{76.5}  & \textbf{86.6} & \textbf{45.0} & \textbf{76.4}  & \textbf{87.3} & 36.3 &62.8 & 71.7 &\textbf{14.1} & 26.6 & 33.5 & 23.3  \\ 

\hlineB{3}
\end{tabular}
} \label{ablation_iter}
} \hfill

\subfloat[LLM assessment results by using GPT4 as a reference. RG: ROUGE score \cite{rouge}; BERT: BERTScore-F1 \cite{bertscore}; Time: Average running time on one summarization task. The model underlined is the final selected LLM.]
{
\scalebox{1}{
\begin{tabular}{l|cccc|c|l|cccc|c}
\hlineB{3}
LLM            & RG-1 & RG-2 & RG-L & \multicolumn{1}{l|}{BERT} & \multicolumn{1}{l|}{Time (s)} & LLM            & RG-1 & RG-2 & RG-L & \multicolumn{1}{l|}{BERT} & \multicolumn{1}{l}{Time (s)}  \\ \hline
Longchat 7b\cite{longchat}  & 0.43  & 0.20  & 0.34  & 0.90                            & 2.45    & Internlm 7b \cite{internlm}     & 0.32  & 0.13  & 0.26  & 0.87                            & 3.36      \\
OpenLlama 7b \cite{openllama}    & 0.48  & 0.24  & 0.39  & 0.89                            & 1.03   &  RWKV-4 7b \cite{rwkv}     & 0.28  & 0.11  & 0.23  & 0.88                            & 1.04      \\
OpenLlama 13b \cite{openllama}    & 0.38  & 0.18  & 0.31  & 0.90                            & 2.19  & Vicuna 7b \cite{vicuna}       & 0.46  & 0.23  & 0.37  & 0.91                            & 1.91                                                         \\
Fastchat t5 3b\cite{fastchatt5}  & 0.48  & 0.25  & 0.40  & 0.91                            & 2.97      &  \underline{Vicuna 13b} \cite{vicuna}      & 0.48  & 0.24  & 0.39  & 0.92                            & 2.19                 \\
Dolly-v2-7b \cite{dolly}         & 0.36  & 0.15  & 0.28  & 0.89                            & 4.93  & Vicuna 33b \cite{vicuna}     & 0.50  & 0.27  & 0.42  & 0.92                            & 7.38  \\ \hlineB{3}

\end{tabular}
}\label{ablation_llm}
}

\end{table*}
% \begin{table*}[t]
% \centering

% \caption{Ablation finetuning results on ActivityNet Captions text-to-video retrieval dataset, the number of iterations are set to $1$ for both video and text branches.}
% \end{table*}


% \label{ablation_anet}
% \caption{Ablation finetuning results on ActivityNet Captions text-to-video retrieval dataset with different setups of pretraining the encoders. The number of iterations are set to $3$ for both video and text branches.}

==> sec/tables/ablation_iter.tex <==
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{c|ccc|ccc|ccc|ccc|c}
\hlineB{3}
\#iter & \multicolumn{3}{c|}{FT A-Net T2V} & \multicolumn{3}{c|}{FT A-Net V2T} & \multicolumn{3}{c|}{ZS MSRVTT T2V} & \multicolumn{3}{c|}{ZS LSMDC T2V} & ZS C-Ego\\
Video-Text                   & R@1 & R@5 & R@10 & R@1 & R@5 & R@10  &R@1 & R@5 & R@10 &R@1 & R@5 & R@10 &mAP \\ \hline
1-1                      & 43.1     & 73.2     & 84.5     & 42.6     & 73.4     & 84.8  & \textbf{37.3} &\textbf{63.8} & \textbf{72.5} &12.9 & \textbf{28.3} & \textbf{35.5} &22.9 \\ 
3-1                      & 44.8     & 75.5     & 86.0 & 44.7 & 75.4     & 86.5  & 36.3 &62.5 & 72.1 &13.8 & 27.7 & 35.3 &   \textbf{23.4}  \\       
3-3                      & \textbf{45.3}& \textbf{76.5}  & \textbf{86.6} & \textbf{45.0} & \textbf{76.4}  & \textbf{87.3} & 36.3 &62.8 & 71.7 &\textbf{14.1} & 26.6 & 33.5 & 23.3  \\ 

\hlineB{3}
\end{tabular}

\caption{Ablation study results on the number of iterations across different datasets and scenarios, finetuning (FT) and zero-shot (ZS). A-Net: ActivityNet Captions; C-Ego: Charades-Ego.}
\end{table*}





% \begin{table}[]
% \centering
% \begin{tabular}{c|c|c}
% \hline
% PT Setup          & \begin{tabular}[c]{@{}c@{}}\#Video-Text Iterations\end{tabular} & mAP  \\ \hline
% Data1             & 2-2                                                                         & 22.9 \\ \hline
% Data1+Data2       & 4-4                                                                         & 22.7 \\ \hline
% Data1+Data2+Data3 & 4-2                                                                         & 23.4 \\ \hline
% \end{tabular}
% \label{ablation_charades}
% \caption{Ablation zero-shot results on Charades-Ego action recognition dataset.}
% \end{table}



% PT Setup                                                                      & \begin{tabular}[c]{@{}c@{}} \#Video-Text Iterations\end{tabular} & R@1 & R@5 & R@10 & R@1 & R@5 & R@10  \\ \hline
% SVST                                                                         & 2-2 & 41.6     & 72.8     & 83.7      & 41.2     & 72.6     & 84.0       \\ \hline
% \multirow{2}{*}{SVST+LVLT}                                                  & 2-2 & 42.8     & 72.8     & 84.0      & 41.8     & 73.0     & 84.3         \\
%                                                                               & 4-4 & 44.7     & 74.9     & 85.7       & 43.1     & 74.9     & 86.2  \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}SVST+LVLT+LVST\end{tabular}}        & 2-2 & 43.1     & 73.2     & 84.5     & 42.6     & 73.4     & 84.8        \\
%                                                                               & 4-2 & 44.8     & 75.5     & 86.0        & \textbf{44.7}     & 75.4     & 86.5           \\
%                                                                               & 4-4 & \textbf{45.2}     & \textbf{75.9}     & \textbf{86.2}       & 44.0     & \textbf{76.0}     & \textbf{86.9}       \\ \hline
% \end{tabular}
% \label{ablation_anet}
% \caption{Ablation finetuning results on ActivityNet Captions text-to-video retrieval dataset, the number of iterations are set to $1$ for both video and text branches.}
% \end{table*}

==> sec/tables/ablation_llm.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{l|cccc|c|l|cccc|c}
\hlineB{3}
LLM            & RG-1 & RG-2 & RG-L & \multicolumn{1}{l|}{BERT} & \multicolumn{1}{l|}{Time (s)} & LLM            & RG-1 & RG-2 & RG-L & \multicolumn{1}{l|}{BERT} & \multicolumn{1}{l}{Time (s)}  \\ \hline
Longchat 7b\cite{longchat}  & 0.43  & 0.20  & 0.34  & 0.90                            & 2.45    & Internlm-7b \cite{internlm}     & 0.32  & 0.13  & 0.26  & 0.87                            & 3.36      \\
Open-llama 7b \cite{openllama}    & 0.48  & 0.24  & 0.39  & 0.89                            & 1.03   &  RWKV-4-7b \cite{rwkv}     & 0.28  & 0.11  & 0.23  & 0.88                            & 1.04      \\
Open-llama 13b \cite{openllama}    & 0.38  & 0.18  & 0.31  & 0.90                            & 2.19  & Vicuna 7b \cite{vicuna}       & 0.46  & 0.23  & 0.37  & 0.91                            & 1.91                                                         \\
Fastchat t5-3b\cite{fastchatt5}  & 0.48  & 0.25  & 0.40  & 0.91                            & 2.97      &  \textbf{Vicuna 13b} \cite{vicuna}      & 0.48  & 0.24  & 0.39  & 0.92                            & 2.19                 \\
Dolly-v2-7b \cite{dolly}         & 0.36  & 0.15  & 0.28  & 0.89                            & 4.93  & Vicuna 33b \cite{vicuna}     & 0.50  & 0.27  & 0.42  & 0.92                            & 7.38  \\ \hlineB{3}

 
\end{tabular}
\caption{LLM verification results by using GPT4 as a reference. RG: ROUGE score \cite{rouge}; BERT: BERTScore-F1 \cite{bertscore}; Time: Average running time on one summarization task.}
\end{table}

==> sec/tables/ablation_way_pretraining.tex <==
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{l|ccc|ccc}
\hlineB{3}
\multirow{2}{*}{Encoder PT Setup} & \multicolumn{3}{c|}{T2V} & \multicolumn{3}{c}{V2T}\\
                         & R@1 & R@5 & R@10 & R@1 & R@5 & R@10  \\ \hline
Scratch                  & 24.7     & 51.1     & 64.1      & 24.7     & 52.6     & 65.9       \\ 
Fixed CLIP weights       & 37.5     & 67.4     & 80.6      & 36.9     & 68.0     & 80.9         \\                 
CLIP weights, smaller LR & \textbf{45.3}     & \textbf{76.5}     & \textbf{86.6}     & \textbf{44.5}     & \textbf{76.4}     & \textbf{87.3}        \\
\hlineB{3}
\end{tabular}
\caption{Ablation finetuning results on ActivityNet Captions text-to-video retrieval dataset with different setups of pretraining the encoders. The number of iterations are set to $3$ for both video and text branches.}
\end{table*}

==> sec/tables/activitynet.tex <==
%\begin{table*}[t]
%\centering
%\begin{tabular}{l|cccccc}
%\hline
%\multirow{2}{*}{Method}                       &\multicolumn{5}{c}{T2V Finetune}         \\ \cline{2-6} 
%                                   & Pretraining data             & R@1  & R@5   & R@10  & R@50  & MedR \\ \hline
%CLIPBert\cite{clipbert}            &             & 21.3 & 49.0  & 63.5  & -     & 6.0  \\
%Frozen\cite{frozen}                &             & 28.8 & 60.9  & -     & -     & 3.0  \\
%TACo\cite{taco}                    &             & 30.4 & 61.2  & -     & 93.4  & 3.0  \\
%PerceiverVL\cite{perceivervl}      &             & 33.9 & 62.1  & 76.4  & -     & -     \\
%LF-VILA\cite{lfvila}               &             & 35.3 & 65.4  & -     & 95.0  & 3.0  \\
%CLIP4Clip-meanP\cite{clip4clip}    &             & 40.5 & 72.4  & -     & 98.1  & \textbf{2.0}  \\
%X-CLIP(B/32)\cite{xclip}           &             & 44.3 & 74.1  & -     & -  & -  \\
%Ours                               &             & \textbf{45.2} & \textbf{75.9}  & \textbf{86.2}  & \textbf{98.2}  & \textbf{2.0}   \\
%X-CLIP(B/16)                       &             & 46.2 & 75.5  & -  & -  & -   \\
%CenterCLIP(B/16)                   &             & 46.2 & 77.0  & 87.6  & -  & 2.0\\
%DMAE & & 44.8 & 74.4 & 85.1 & - & 2.0 \\
%ViCLIP & & & & & & \\

%46.2	77.0	87.6
%\hline
%\end{tabular}
%\label{activitynet_table}
%\caption{Finetuning results on ActivityNet Captions text-to-video retrieval dataset.}
%\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\begin{tabular}{@{}lllcccccccc@{}}
\hlineB{3}
\multirow{2}{*}{Method}          &  \multirow{2}{*}{\#PT} &  \multirow{2}{*}{Model}        & \multicolumn{4}{c}{T2V}       & \multicolumn{4}{c}{V2T}   \\
                                           &   &  & R@1           & R@5           & R@10          & MdR  & R@1           & R@5           & R@10          & MdR                         \\ \hlineB{2}
\multicolumn{11}{l}{\textit{Zero-shot}}  \\ 
ViCLIP\cite{internvid} & 10M        & ViT$_{L14}$     & 15.1          & -          & -            & -  &24.0  &-  &-  &- \\ 
Ours                            & 10M       & ViT$_{B32}$  & 35.3 &64.3  &76.1  &3.0  & 35.0 &64.9  &77.6  &3.0 \\\hlineB{2}
\multicolumn{11}{l}{\textit{Finetuning}}  \\
CLIPBert\cite{clipbert}         & 5.6M      & Res$_{50}$ & 21.3          & 49.0          & 63.5               & 6.0   &-  &-  &- &-     \\
TACo\cite{taco}                 & 100M      & Res$_{152}$ & 30.4          & 61.2           &-             & 3.0   &-  &-  &-  &-    \\
Per-VL\cite{perceivervl}   & 5.5M      & ViT$_{B32}$  & 33.9          & 62.1          & 76.4                  & -    &-  &-  &-  &-    \\
C4c-mP\cite{clip4clip} & 100M      & ViT$_{B32}$  & 40.5          & 72.4          & -                 & 2.0 &42.5  &74.1  &85.8  &\textbf{2.0}      \\
Ours                            & 10M       & ViT$_{B32}$  & \textbf{45.3} & \textbf{76.5} & \textbf{86.6} & \textbf{2.0} & \textbf{45.0} & \textbf{76.4} & \textbf{87.3}  & \textbf{2.0} \\ \hlineB{2}

\rowcolor{gray!10}

X-CLIP\cite{xclip}        & -         & ViT$_{B32}$  & 44.3          & 74.1          & -                     & -  &43.9  &73.9  &-  &-       \\
\rowcolor{gray!10}

X-CLIP\cite{xclip}                    & -         & ViT$_{B16}$  & 46.2          & 75.5               & -              & -  &46.4  &75.9  &-   & -      \\
\rowcolor{gray!10}
CenCLIP \cite{centerclip}                & -         & ViT$_{B16}$  & 46.2          & 77.0          & 87.6              & 2.0 &46.7  &77.1  &88.0  & 2.0      \\ 
\rowcolor{gray!10}
Frozen\cite{frozen}             & 5.5M      & TS4mer & 28.8          & 60.9          & -                & 3.0   &-  &-  &-  &-      \\
\rowcolor{gray!10}
LF-VILA\cite{lfvila}            & 60M       & Swin$_B$    & 35.3          & 65.4          & -                   & 3.0  &-  &-  &-  &-      \\
\rowcolor{gray!10}
HiTeA\cite{hitea}                          & 5M        & MViT$_B$    & 45.1          & 73.5          & 84.2                  & -  &-  &-  &-  &-    \\
\rowcolor{gray!10}
ViCLIP \cite{internvid} & 10M        & ViT$_{L14}$     & 49.8          & -             & -    & -  &48.1  &-  &- &- \\ \hlineB{3}
\end{tabular}
\label{activitynet_table}
\caption{Text-to-video and video-to-text retrieval results on ActivityNet Captions dataset.}
\end{table*}

==> sec/tables/charades-ego.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{lccc}
\hlineB{3}
Method  & ZS mAP & FT mAP & $\Delta_{\text{FT-ZS}}$ \\ \hline
Actor \cite{actor}             & -     & 20.0 &-\\
SSDA \cite{ssda}               & -     & 23.1 &-\\
I3D \cite{ssda}                & -     & 25.8 &-\\
Ego-Exo \cite{egoexo}                       & -     & 30.1 &-\\
EgoVLP \cite{egovlp}           & 25.0  & 32.1 &7.1\\
HierVL-Avg \cite{hiervl}       & 25.2  & 32.6 &7.4 \\ 
HierVL-SA \cite{hiervl}        & \textbf{26.0}  & \textbf{33.8} &7.8 \\ 
% EgoVLPv2 \cite{egovlpv2}       & 26.2  & 34.1 &7.9 \\
Ours                          & 23.4  & \underline{33.7} &\textbf{10.3} \\ \hlineB{3}
\end{tabular}
\label{charades_ego_table}
\caption{Video Action Classification results on Charades-Ego dataset.}
\end{table}

==> sec/tables/coin.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{lcc}
\hlineB{3}
Method    & \#PT Data   & Accuracy \\ \hline
CLIPBert \cite{clipbert} &  5.6M  & 65.4     \\
SlowFast \cite{slowfast} &  100M & 71.6     \\
VideoCLIP \cite{videoclip} &  100M    & 72.5 \\
Ours        &  10M   & \textbf{84.8}     \\ \hline
\rowcolor{gray!10} TS4mer \cite{timesformer} & 0.37M & 83.5  \\
\rowcolor{gray!10} TS4mer \cite{timesformer} & 100M & 85.3  \\
\rowcolor{gray!10} LF-VILA \cite{lfvila}    &  60M & 85.7     \\ \hlineB{3}
\end{tabular}
\label{coin_table}
\caption{Video classification results on COIN dataset.}
\end{table}

==> sec/tables/lsmdc.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lcccccccc}
\hlineB{3}
\multirow{2}{*}{Method}                         & \multicolumn{4}{c}{T2V} & \multicolumn{4}{c}{V2T}         \\ 
                                                & R@1  & R@5   & R@10  & MdR& R@1  & R@5   & R@10  & MdR \\ \hline
\multicolumn{9}{l}{\textit{Zero-Shot}}  \\ 
Frozen-ZS\cite{frozen}                    & 13.6 & 27.9  & 33.5    & 32.0  &-&-&-&- \\
CLIP4Clip-meanP-ZS\cite{clip4clip}        & 15.1 & 28.5  & 36.4    & 28.0  & -  & - & -  & \\
ViCLIP-ZS\cite{internvid}                 & 20.1 & -  & -    & -   &16.9 & - & - & - \\
Ours-ZS                                   & 12.9  & 28.3 &  35.1 &  35.5     & 13.0 &  26.8 & 33.9   & 43.0 \\ \hline
\multicolumn{9}{l}{\textit{Comparable Finetuning}}  \\ 
PerceiverVL\cite{perceivervl}                   & 15.8 & 37.6  & 40.1    & -     &-&-&-&- \\
CLIP4Clip-meanP\cite{clip4clip}                 & 20.7 & 38.9  & 47.2    & 13.0  &20.6 & 39.4 & 47.5 & 13.0 \\
Ours                                            & \textbf{21.2} & \textbf{40.9}  & \textbf{51.4}    & \textbf{9.0} & \textbf{21.9} & \textbf{40.5}  & \textbf{50.2}    & \textbf{10.0} \\ \hline

\multicolumn{9}{l}{\textit{Retrieval Only}}  \\ 

X-CLIP(B/32)\cite{xclip}                         & 23.3 & 43.0  & -       & -     &22.5 & 42.2 & - & - \\
X-CLIP(B/16)\cite{xclip}                         & 26.1 & 48.4  & -       & -     &26.9 & 46.2 & - & - \\
CenterCLIP\cite{centerclip}                     & 24.2 & 46.2  & 55.9    & 8.0   &24.5 & 46.4 & 55.8 & 7.0 \\ \hline
\multicolumn{9}{l}{\textit{Higher Backbone FLOPs} \cite{flops}}\\ 
Frozen\cite{frozen}                             & 15.0 & 30.8  & 40.3    & 20.0  &-&-&-&- \\
HiTeA\cite{centerclip}                          & 27.1 & 46.2  & 54.5    & -     & -   & - & - & - \\
ViCLIP\cite{internvid}                          & 33.0 & -  & -    & -   &32.5 & - & - & - \\ \hlineB{3}
\end{tabular}
\label{lsmdc_table}
\caption{Text-to-video and video-to-text retrieval results on LSMDC dataset.}
\end{table*}

==> sec/tables/msrvtt.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lcccccccc}
\hlineB{3}
\multirow{2}{*}{Method}                         & \multicolumn{4}{c}{T2V}  & \multicolumn{4}{c}{V2T}    \\
                                                & R@1  & R@5   & R@10 & MdR & R@1  & R@5   & R@10 & MdR\\ \hline
\multicolumn{9}{l}{\textit{Zero-Shot}}  \\
Frozen-ZS\cite{frozen}                    & 24.7 & 46.9  & 57.2  & 3.0  &-&-&-&-\\
CLIP4Clip-meanP-ZS\cite{clip4clip}        & 32.0 & 57.0  & 66.9  & 4.0 &-  &-  &-  &-  \\    
ViCLIP-ZS\cite{internvid}                 & 42.4 & -     & -     & -   &41.3&-   &-   &-  \\
Ours-ZS                                   & 37.3 & 63.8   & 72.5   & 3.0  &39.5& 64.6 & 73.0 & 2.0  \\ \hline
\multicolumn{9}{l}{\textit{Comparable Finetuning}}  \\ 
CLIPBert\cite{clipbert}                         & 21.3 & 49.0  & 63.5  & 6.0 &-&-&-&- \\
TACo\cite{taco}                                 & 24.5 & 52.8  & 65.5  & 5.0  &-&-&-&-\\       
PerceiverVL\cite{perceivervl}                   & 32.6 & 62.1  & 71.6  & -   &-&-&-&-\\
CLIP4Clip-meanP\cite{clip4clip}                 & 43.1 & 70.4  & 80.8  & 2.0 &43.1&70.5&81.2&2.0  \\
Ours                                            &\textbf{46.8} & \textbf{72.0}  & \textbf{81.5}  & \textbf{2.0} & \textbf{47.4} & \textbf{74.0}  & \textbf{81.8}  & \textbf{2.0}  \\ \hline
\multicolumn{9}{l}{\textit{Retrieval Only}}  \\ 

X-CLIP(B/32)\cite{xclip}                        & 46.1 & 73.0  & 83.1  & 2.0 &46.8&73.3&84.0&2.0  \\    
X-CLIP(B/16)\cite{xclip}                        & 49.3 & 75.8  & 84.8  & 2.0 &48.9&76.8&84.5&2.0  \\  
CenterCLIP(B/16)\cite{centerclip}               & 48.4 & 73.8  & 82.0  & 2.0 &47.7&75.0&83.3&2.0  \\ \hline 

\multicolumn{9}{l}{\textit{Higher Backbone FLOPs} \cite{flops}}  \\ 
Frozen\cite{frozen}                             & 32.5 & 61.5  & 71.2  & 3.0  &-&-&-&-\\
HiTeA\cite{hitea}                               & 44.4 & 69.3  & 78.9  & 2.0 &-   &-   &-   &-  \\
ViCLIP\cite{internvid}                          & 52.5 & -     & -     & -   &51.8&-   &-   &-  \\ \hlineB{3}


\hline
\end{tabular}
\label{msrvtt_table}
\caption{Text-to-video and video-to-text retrieval results on MSR-VTT dataset.}
\end{table*}

==> sec/tables/pt_iter_setup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\hlineB{3}
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}PT Video-Text\\ $\#iter$ setup\end{tabular}} & \multicolumn{3}{c|}{A-Net T2V} & \multicolumn{3}{c|}{A-Net V2T} & \multicolumn{3}{c|}{MSRVTT T2V} & \multicolumn{3}{c}{MSRVTT V2T} \\
& R@1      & R@5      & R@10     & R@1      & R@5      & R@10   & R@1       & R@5      & R@10     & R@1      & R@5      & R@10  \\ \hlineB{1}
Only 1-1(sub) & 35.2     & 63.9     & 75.6     & 34.4     & 63.6     & 76.6  &  36.6      & 63.5     & 72.3     & 39.8     & 63.5     & 72.3    \\ 
Only 3-3(sub) & 35.0     & 64.0     & 76.2     & 34.0     & 64.1     & 76.4  & 36.7      & \textbf{64.8}     & 72.3     & \textbf{40.0}     & 64.3     & \textbf{73.4}  \\
1-1\&3-1\&3-3  & \textbf{35.3}     & \textbf{64.3}     & \textbf{76.3}     & \textbf{35.0}     & \textbf{64.9}     & \textbf{77.6}    & \textbf{37.3}      & 63.8     & \textbf{72.5}     & 39.5     & \textbf{64.6}     & 73.0  \\ \hlineB{3}

% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}PT Video-Text\\ $\#iter$ setup\end{tabular}} 


% Only 1-1(sub) 
% Only 3-3(sub) 
% 1-1\&3-1\&3-3 


\end{tabular}
\caption{Zero-shot retrieval results across different pre-training $\#iter$ setups. PT: Pretraining; A-Net: ActivityNet Captions.}
\label{supple_iter}
\end{table*}

==> sec/tables/retrieval_v2t.tex <==
%\begin{table*}[t]
%\centering
%\begin{tabular}{l|cccccc}
%\hline
%\multirow{2}{*}{Method}                       &\multicolumn{5}{c}{T2V Finetune}         \\ \cline{2-6} 
%                                   & Pretraining data             & R@1  & R@5   & R@10  & R@50  & MedR \\ \hline
%CLIPBert\cite{clipbert}            &             & 21.3 & 49.0  & 63.5  & -     & 6.0  \\
%Frozen\cite{frozen}                &             & 28.8 & 60.9  & -     & -     & 3.0  \\
%TACo\cite{taco}                    &             & 30.4 & 61.2  & -     & 93.4  & 3.0  \\
%PerceiverVL\cite{perceivervl}      &             & 33.9 & 62.1  & 76.4  & -     & -     \\
%LF-VILA\cite{lfvila}               &             & 35.3 & 65.4  & -     & 95.0  & 3.0  \\
%CLIP4Clip-meanP\cite{clip4clip}    &             & 40.5 & 72.4  & -     & 98.1  & \textbf{2.0}  \\
%X-CLIP(B/32)\cite{xclip}           &             & 44.3 & 74.1  & -     & -  & -  \\
%Ours                               &             & \textbf{45.2} & \textbf{75.9}  & \textbf{86.2}  & \textbf{98.2}  & \textbf{2.0}   \\
%X-CLIP(B/16)                       &             & 46.2 & 75.5  & -  & -  & -   \\
%CenterCLIP(B/16)                   &             & 46.2 & 77.0  & 87.6  & -  & 2.0\\
%DMAE & & 44.8 & 74.4 & 85.1 & - & 2.0 \\
%ViCLIP & & & & & & \\

%46.2	77.0	87.6
%\hline
%\end{tabular}
%\label{activitynet_table}
%\caption{Finetuning results on ActivityNet Captions text-to-video retrieval dataset.}
%\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
\centering
\footnotesize
\caption{Video-to-text (V2T) retrieval results using Recall at K (R@K) and Median Rank (MdR) metrics across different setups for ActivityNet Captions, MSR-VTT, and LSMDC datasets. Results for models that are not directly comparable due to differences in setups are shown in gray. \#PT represents the size of the pretraining dataset.}
\vspace{-1mm}
\scalebox{0.72}{
\begin{tabular}{@{}llll|cccc|cccc|cccc@{}}
\hlineB{3}
\multirow{2}{*}{Video-to-text (V2T) Setup} & \multirow{2}{*}{Method} &  \multirow{2}{*}{\#PT} &  \multirow{2}{*}{Backbone}    & \multicolumn{4}{c|}{ActivityNet Captions V2T} & \multicolumn{4}{c|}{MSR-VTT V2T} &\multicolumn{4}{c}{LSMDC V2T} \\

                       & &  &  & R@1   & R@5  & R@10   & MdR  & R@1     & R@5    & R@10 & MdR  & R@1    & R@5  & R@10   & MdR  \\ \hlineB{2}
 
% \multicolumn{3}{l|}{\textit{Zero-shot}} & \multicolumn{4}{l|}{} & \multicolumn{4}{l|}{} & \multicolumn{4}{l}{}   \\
\multirow{2}{*}{Zero-shot} & ViCLIP\cite{internvid}             & 10M & ViT$_{L14}$  & 24.0  &-      &-      &-      & 41.3  &   -   & -     &-      &16.9   & -     & -     & -     \\ 

&Ours                       & 10M & ViT$_{B32}$  & 35.0  &64.9   &77.6   &3.0    & 39.5  & 64.6  & 73.0  &2.0    &13.0   & 26.8  & 33.9  & 43.0  \\

&VideoPrism~\cite{videoprism}                 & 618M & ViViT$_B$  & 47.9  &75.0  &-   &-    & 50.2  & 73.2  & -  &-    &-   & -  & -  & -  \\ \hlineB{2}
% \multicolumn{3}{l|}{\textit{Finetuning, Model with Similar FLOPs}} & \multicolumn{4}{l|}{} & \multicolumn{4}{l|}{} & \multicolumn{4}{l}{}   \\
Finetuned & CLIP4Clip*~\cite{clip4clip}       &136M & ViT$_{B32}$  & 42.5  & 74.1  & 85.8  & 2.0   & 43.1  & 70.5  & 81.2  &2.0    &20.9   & \textbf{40.7}  & 49.1  & 11.0  \\

Model with Similar FLOPs & Ours                             & 10M & ViT$_{B32}$  & \textbf{45.0} & \textbf{76.4} & \textbf{87.3} & \textbf{2.0} & \textbf{47.4} & \textbf{74.0} & \textbf{81.8}  & \textbf{2.0} &\textbf{21.9} &40.5 &\textbf{50.2} &\textbf{10.0} \\ \hlineB{2}

% \multicolumn{3}{l|}{\textit{Finetuning, Retrieval-specific Model}} & \multicolumn{4}{l|}{} & \multicolumn{4}{l|}{} & \multicolumn{4}{l}{}   \\

\rowcolor{gray!10}
&X-CLIP\cite{xclip}                 & -   & ViT$_{B32}$  & 43.9  & 73.9  & -     & -     &46.8   &73.3   &84.0   &2.0    &22.5   &42.2   &-      &-      \\

\rowcolor{gray!10}
Finetuned &PromptSwitch \cite{promptswitch}                 & -   & ViT$_{B32}$  & -  & -  & -     & -     &46.0   &74.3   &84.8   &-    &22.0   &40.8   &50.3      &-       \\

\rowcolor{gray!10}
&UCOFIA\cite{ucofia}                 & -   & ViT$_{B32}$  & 46.3  & 76.5  & -     & -     &47.1   &74.3   &-   &-    &-   &-   &-      &-      \\

\rowcolor{gray!10}
Retrieval-specific Model & X-CLIP\cite{xclip}                 & -   & ViT$_{B16}$  & 46.4  & 75.9  & -     & -     &48.9   &76.8   &84.5   &2.0    &26.9   &46.2   &-      &-       \\

\rowcolor{gray!10}
&CenterCLIP \cite{centerclip}       & -   & ViT$_{B16}$  & 46.7  & 77.1  & 88.0  & 2.0   &47.7   &75.0   &83.3   &2.0    &24.5   &46.4   &55.8   &7.0     \\ \hlineB{1}

% \multicolumn{3}{l|}{\textit{Finetuning, Model with Higher FLOPs}} & \multicolumn{4}{l|}{} & \multicolumn{4}{l|}{} & \multicolumn{4}{l}{}   \\
% \rowcolor{gray!10}
% VideoPrism \cite{videoprism}            & 618M & ViViT$_{B}$ & 47.9   & 75.0     & -     & -     &50.2   &73.2      &-      &-      &-   &-      &-      &-\\

\rowcolor{gray!10}
Finetuned, Higher FLOPs& ViCLIP \cite{internvid}            & 10M & ViT$_{L14}$  & 48.1  & -     & -     & -     &51.8   &-      &-      &-      &32.5   &-      &-      &-\\ \hlineB{3}
\end{tabular}
}
\vspace{-5mm}
\label{v2t}
\end{table*}
